MI-BMInet: An Efficient Convolutional Neural Network for Motor Imagery Brain--Machine Interfaces with EEG Channel Selection

A brain--machine interface (BMI) based on motor imagery (MI) enables the control of devices using brain signals while the subject imagines performing a movement. It plays a vital role in prosthesis control and motor rehabilitation. To improve user comfort, preserve data privacy, and reduce the system's latency, a new trend in wearable BMIs is to execute algorithms on low-power microcontroller units (MCUs) embedded on edge devices to process the electroencephalographic (EEG) data in real-time close to the sensors. However, most of the classification models present in the literature are too resource-demanding, making them unfit for low-power MCUs. This paper proposes an efficient convolutional neural network (CNN) for EEG-based MI classification that achieves comparable accuracy while being orders of magnitude less resource-demanding and significantly more energy-efficient than state-of-the-art (SoA) models for a long-lifetime battery operation. To further reduce the model complexity, we propose an automatic channel selection method based on spatial filters and quantize both weights and activations to 8-bit precision with negligible accuracy loss. Finally, we implement and evaluate the proposed models on leading-edge parallel ultra-low-power (PULP) MCUs. The final 2-class solution consumes as little as 30 uJ/inference with a runtime of 2.95 ms/inference and an accuracy of 82.51% while using 6.4x fewer EEG channels, becoming the new SoA for embedded MI-BMI and defining a new Pareto frontier in the three-way trade-off among accuracy, resource cost, and power usage.

==> 02_figures/D_cs_data.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%% edgeeegnet physionet %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% 4 class physionet












% 3 class physionet












% 2 class physionet












%%%%%%%%%%%%%%%%%%%%%%%%%%%% eegnet physionet %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% 4 class physionet












% 3 class physionet












% 2 class physionet












%%%%%%%%%%%%%%%%%%%%%%%%%%%%% bci comp iv 2a  %%%%%%%%%%%%%%%%%%%

% edgeeegnet





















%% 3 class





















%% 2 class





















% % eegnet  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{filecontents*}{eegn-bci-auto.dat}
% x y 
% 2 47.21326853934674
% 3 54.010662925127704
% 4 59.90395629297916
% 5 63.111758204391506
% 6 67.73829876552348
% 7 67.96565776981689
% 8 68.02333751209312
% 9 66.32638205734595
% 10 67.35511817212547
% 11 70.8713801701427
% 14 69.62149855223252
% 16 70.74354572553986
% 18 69.74204811387042
% 19 70.1689353018756
% 20 71.41064889572384
% \end{filecontents*}

% \begin{filecontents*}{eegn-bci-full.dat}
% x y 
% 2 70.4038241354052
% 20 70.4038241354052
% \end{filecontents*}





==> 02_figures/T_bcicompiv2aResComparison.tex <==

%\setlength{\tabcolsep}{2.7pt}
\begin{table*}[!b]
\renewcommand{\arraystretch}{1.1}
\caption{Classification accuracy (\%), number of parameters, memory footprint of the two largest consecutive feature maps, and computational complexity of \edgeeegnet{} and its comparison with related works on the BCI Competition IV-2a dataset. Parameters, memory, and MACC are reported for the 2-class case if not stated otherwise. The best solution for each configuration and metric is marked in bold.}
\centering
\label{tab:bciResComp}
{
  \begin{threeparttable}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
          & \multirow{2}[3]{*}{\begin{tabular}[c]{@{}r@{}}Tot. \#\\ params\end{tabular}} & \multirow{2}[3]{*}{\begin{tabular}[c]{@{}r@{}}Max. feature\\ map size\end{tabular}} & \multirow{2}[3]{*}{\begin{tabular}[c]{@{}r@{}}Tot. \#\\ MACC\end{tabular}} & \multicolumn{3}{c}{Accuracy/Kappa}                     \\ \cmidrule(l){5-7} 
          & &  & & \multicolumn{1}{r}{2-}   & \multicolumn{1}{r}{3-}    & \multicolumn{1}{r}{4-class}  \\ 
%\cmidrule{1-2} \cmidrule{3-5} \cmidrule(l){6-8} 
\midrule
\#\,ch = 22 \\
%\hspace{1mm} FBCSP~\cite{abbas2018biocas} & - & - & - & -\,/\,- & -\,/\,- & -\,/\,0.59 \\
\hspace{1mm} FBCSP~\cite{das2020fbcspovr} & - & - & - & -\,/\,- & -\,/\,- & -\,/\,0.65 \\
%RoCSP-SRIT2NFIS~\cite{das2016bcifuzzy} & 22 & - & - & - & 83.26\,/\,- & -\,/\,- & -\,/\,- \\
%\hspace{1mm} FBCSP~\cite{Hersche2018FastFeatures} & 50.0\,k & 49\,k & - & -\,/\,- & -\,/\,- & 74.77\,/\,- \\
%\hspace{1mm} CSP~\cite{Hersche2018FastFeatures} & 261\,k & 50\,k & 104\,M & -\,/\,- & -\,/\,- & 73.70\,/\,- \\
\hspace{1mm} MRC~\cite{Hersche2018FastFeatures} & - & - & - & -\,/\,- & -\,/\,- & 75.47\,/\,- \\
\hspace{1mm} MSFBCNN~\cite{wu2019_MSFBCNN} & 155\,k & 5,775\,k & 202\,M & -\,/\,- & -\,/\,- & 75.80\,/\,- \\
\hspace{1mm} FB+3D-CNN~\cite{bang2021fb3dcnn} & - & - & - & \textbf{86.96}\,/\,- & -\,/\,- & -\,/\,- \\
\hspace{1mm} S. ConvNet~\cite{Schirrmeister2017DeepVisualization}$^\dagger$ & 47.3\,k & 1,013\,k & 63.0\,M & 79.90\,/\,- & -\,/\,- & 74.31\,/\,0.66 \\
\hspace{1mm} EEG-TCNet (fixed)~\cite{ingolfsson2020eegtcnet} & 4.27\,k & 396\,k & 6.8\,M & -\,/\,- & -\,/\,- & \textbf{77.35\,/\,0.70} \\
\hspace{1mm} E-CSP~\cite{das2015smcconf} & - & - & - & 80.56\,/\,- & -\,/\,- & -\,/\,- \\
\hspace{1mm} CSP+Riemannian~\cite{chen2020cssimilarity} & - & - & - & -\,/\,- & -\,/\,- & 75.57\%\,/\,0.67 \\
\hspace{1mm} \acrshort{wola}\acrshort{csp}~\cite{belwafi2018_wolacsp} & - & - & - & 78.85\,/\,- & -\,/\,- & -\,/\,- \\
\hspace{1mm} \acrshort{csp}+\acrshort{svm}~\cite{malekmohammadi2019_cspsvm} & - & - & - & 80.55\,/\,- & -\,/\,- & 67.21\,/\,-  \\
\hspace{1mm} EEGNet~\cite{Lawhern2018EEGNet:Interfaces}$^*$ & \textbf{2.63\,k} & 223\,k & 12.98\,M & -\,/\,- & -\,/\,- & 71.30\,/\,- \\
\hspace{1mm} \edgeeegnet{} (proposed) & 4.92\,k & \textbf{40.5\,k} & \textbf{2.16\,M} & 86.32\,/\,0.73 & 80.37\,/\,0.71 & 76.03\,/\,0.68 \\
%\midrule
\#\,ch = 14 \\
\hspace{1mm} \edgeeegnet{} & - & - & - & 86.80\,/\,0.74 & \textbf{80.54\,/\,0.71} & 75.84\,/\,0.68 \\
%\edgeeegnet{} & 16 & - & - & - & 86.65\,/\,0.73 & 80.86\,/\,0.71 & 76.57\,/\,0.69 \\
%\#\,ch = 17.67$^*$ \\
Subject-specific \\
\hspace{1mm} \edgeeegnet{} (\#\,ch = 13.22$^\ddagger$) & - & - & - & 87.65\,/\,0.75 & -\,/\,- & -\,/\,- \\
\hspace{1mm} \edgeeegnet{} (\#\,ch = 17.44$^\ddagger$) & - & - & - & -\,/\,- & 81.52\,/\,0.72 & -\,/\,- \\
\hspace{1mm} \edgeeegnet{} (\#\,ch = 17.67$^\ddagger$) & - & - & - & -\,/\,- & -\,/\,- & 77.18\,/\,0.70 \\
%\#\,ch = 15.2$^*$ \\
\hspace{1mm} CSP+Riemannian (\#\,ch = 15.2$^\ddagger$)~\cite{chen2020cssimilarity} & - & - & - & -\,/\,- & -\,/\,- & 77.82\,/\,0.71 \\
%CBN+SVM~\cite{he2016bci15ch} & 15 & - & - & - & -\,/\,- & -\,/\,- & -\,/\,0.66 \\
%\midrule
%\edgeeegnet{} & 9 & - & - & - & \,/\, & \,/\, & \,/\, \\
%FSDE~\cite{wang2012subjspecificcsbcicomp} & 8.22$^*$ & - & - & - & -\,/\,0.57 & -\,/\,- & -\,/\,- \\
%\#\,ch = 8.11$^*$ \\
\hspace{1mm} E-CSP (\#\,ch = 8.11$^\ddagger$)~\cite{das2015smcconf} & - & - & - & 83.61\,/\,- & -\,/\,- & -\,/\,- \\
%\hspace{1mm} \edgeeegnet{} & 8 & - & - & - & 85.70\,/\,0.71 & 78.31\,/\,0.67 & 73.55\,/\,0.65 \\
\bottomrule
\end{tabular}
\begin{tablenotes}\footnotesize
\item $^*$ Adapted and deployed by~\cite{Schneider2020}. \hspace{0.5cm} $^\dagger$ Reproduced in~\cite{bang2021fb3dcnn} and in~\cite{ingolfsson2020eegtcnet} for 2- and 4-class tasks, respectively.
\item $^\ddagger$ Averaged over subjects, each of which has different number of selected channels.
\end{tablenotes}
  \end{threeparttable}
  }
\end{table*}


% \setlength{\tabcolsep}{4.7pt}
% \begin{table*}[b]
% \caption{Classification accuracy (\%)\,/\,kappa value with all channels and best accuracy\,/\,kappa value with corresponding subset of selected channels for each subject of BCI Competition IV-2a dataset and comparison with related works.}
% %\caption{Classification accuracy (\%)\,/\,kappa value for each subject of BCI Competition IV-2a dataset with all channels and best number of channels and comparison with related works.}
% \centering
% \label{tab:bciResComp}
% {
% \scriptsize
% \begin{tabular}{@{}lr@{\hspace{\tabcolsep}}rr@{\hspace{\tabcolsep}}rr@{\hspace{\tabcolsep}}rr@{\hspace{\tabcolsep}}rrr@{}}
% \toprule
%         & \multicolumn{4}{c}{2-class}                                                                  & \multicolumn{2}{c}{3-class}                  & \multicolumn{4}{c}{4-class}\\
% \cmidrule(lr){2-5} \cmidrule(lr){6-7} \cmidrule(l){8-11} 
% & \multicolumn{2}{c}{edgeEEGNet} & \multicolumn{2}{c}{CSP and E-CSP~\cite{das2015smcconf}} & \multicolumn{2}{c}{edgeEEGNet} & \multicolumn{2}{c}{edgeEEGNet} & FSDE~\cite{wang2012subjspecificcsbcicomp} & CBN+SVM~\cite{he2016bci15ch} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-10} \cmidrule(l){11-11} 
% S. & all ch. & sel. ch. & all ch. & sel. ch. & all ch. & sel. ch. & all ch. & sel. ch. & sel. ch. & sel. ch. \\
% %\cmidrule{1-1} \cmidrule(l){2-2} \cmidrule(l){3-3} \cmidrule(l){4-4} \cmidrule(l){5-5} \cmidrule(l){6-6} \cmidrule(l){7-7} \cmidrule(l){8-8} \cmidrule(l){9-9} \cmidrule(l){10-10} \cmidrule(l){11-11} 
% \midrule
% 1       & 84.03\,/\,0.681      & 86.98\,/\,0.740\,(4)        & 90.78\,/\,-               & 83.36\,/\,-\,(9)        & 89.43\,/\,0.841      & 91.18\,/\,0.868\,(14)       & 83.10\,/\,0.775      & 84.41\,/\,0.792\,(20)       & -\,/\,0.56\,(8)            & -\,/\,0.69\,(15)                 \\
% 2       & 71.15\,/\,0.423      & 72.65\,/\,0.453\,(20)        & 59.85\,/\,-               & 71.83\,/\,-\,(11)       & 65.74\,/\,0.487      & 68.76\,/\,0.532\,(16)       & 59.27\,/\,0.458      & 60.49\,/\,0.474\,(18)       & -\,/\,0.41\,(11)           & -\,/\,0.51\,(15)                 \\
% 3       & 94.95\,/\,0.899      & 94.95\,/\,0.899\,(22)       & 97.81\,/\,-               & 98.54\,/\,-\,(13)       & 91.67\,/\,0.875      & 92.18\,/\,0.883\,(18)       & 90.64\,/\,0.875      & 90.97\,/\,0.880\,(18)       & -\,/\,0.43\,(6)            & -\,/\,0.87\,(15)                 \\
% 4       & 74.38\,/\,0.488      & 76.66\,/\,0.533\,(9)        & 68.10\,/\,-               & 74.13\,/\,-\,(3)        & 75.66\,/\,0.635      & 76.00\,/\,0.640\,(14)       & 69.77\,/\,0.597      & 70.63\,/\,0.608\,(18)       & -\,/\,0.41\,(9)            & -\,/\,0.85\,(15)                 \\
% 5       & 92.00\,/\,0.839      & 93.84\,/\,0.876\,(4)        & 68.88\,/\,-               & 71.11\,/\,-\,(4)        & 79.17\,/\,0.688      & 80.33\,/\,0.705\,(18)       & 71.83\,/\,0.624      & 73.61\,/\,0.648\,(19)       & -\,/\,0.68\,(3)            & -\,/\,0.78\,(15)                 \\
% 6       & 79.48\,/\,0.590      & 81.11\,/\,0.622\,(20)       & 66.67\,/\,-               & 73.14\,/\,-\,(8)        & 63.48\,/\,0.452      & 65.56\,/\,0.483\,(20)       & 58.10\,/\,0.441      & 59.91\,/\,0.465\,(11)       & -\,/\,0.48\,(12)           & -\,/\,0.42\,(15)                 \\
% 7       & 90.51\,/\,0.810      & 91.17\,/\,0.824\,(20)       & 82.14\,/\,-               & 83.57\,/\,-\,(6)        & 88.49\,/\,0.827      & 88.97\,/\,0.835\,(18)       & 84.71\,/\,0.796      & 85.76\,/\,0.810\,(19)       & -\,/\,0.8\,(11)            & -\,/\,0.54\,(15)                 \\
% 8       & 98.06\,/\,0.961      & 98.27\,/\,0.965\,(6)        & 97.01\,/\,-               & 96.26\,/\,-\,(14)       & 88.18\,/\,0.823      & 88.63\,/\,0.829\,(19)       & 84.55\,/\,0.794 & 86.48\,/\,0.820\,(18)       & -\,/\,0.72\,(3)            & -\,/\,0.97\,(15)                 \\
% 9       & 92.31\,/\,0.846      & 93.26\,/\,0.865\,(14)       & 93.84\,/\,-               & 94.61\,/\,-\,(5)        & 81.53\,/\,0.722      & 82.05\,/\,0.730\,(20)       & 82.33\,/\,0.764 & 82.36\,/\,0.765\,(18)       & -\,/\,0.63\,(11)           & -\,/\,0.45\,(15)                 \\
% %\cmidrule{1-1} \cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7} \cmidrule(l){8-9} \cmidrule(l){10-10} \cmidrule(l){11-11} 
% \midrule
% Avg.    & 86.32\,/\,0.726      & 87.65\,/\,0.753\,(13.22)    & 80.56\,/\,-               & 83.61\,/\,-\,(8.11)     & 80.37\,/\,0.706      & 81.52\,/\,0.723\,(17.44)    & 76.03\,/\,0.680      & 77.18\,/\,0.696\,(17.67)    & -\,/\,0.57\,(8.22)         & -\,/\,0.66\,(15)      \\
% Std.    & 8.96\,/\,0.179        & 8.42\,/\,0.168\,(7.11)      & 14.85\,/\,-                & 11.35\,/\,-\,(3.95)     & 9.78\,/\,0.147        & 9.21\,/\,0.138\,(2.17)      & 11.11\,/\,0.148       & 10.86\,/\,0.145\,(2.45)     & -\,/\,0.15\,(3.29)         & -\,/\,-         \\ \bottomrule
% \end{tabular}
% }
% \end{table*}


% \begin{table}[b]
% \centering
% \caption{Metrics on BCI Competition IV-2a and related works.}
% \label{tab:bciResComp}

% \begin{tabular}{lcrrrr}
% \toprule
% & \begin{tabular}[c]{@{}r@{}}\#\,ch\end{tabular} & \begin{tabular}[c]{@{}r@{}}Tot. \#\\ params\end{tabular} & \begin{tabular}[c]{@{}r@{}}Max. feature\\ map size\end{tabular} & \begin{tabular}[c]{@{}r@{}}Tot. \#\\ MACC\end{tabular} & \begin{tabular}[c]{@{}r@{}}Mean\\ Accuracy\end{tabular} \\
% %\textbf{\begin{tabular}[c]{@{}c@{}}Mean\\ Accuracy\end{tabular}} & \multicolumn{1}{c}{\textbf{Parameters}} & \textbf{\begin{tabular}[c]{@{}c@{}}Mean\\ MACs\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}Feature\\ Map [kB]\end{tabular}}\\ 
% \cmidrule{1-2} \cmidrule{3-6}
% This work & 22 & 4.92\,k & \textbf{43.68\,k} & \textbf{2.16\,M} & 76.03 \\
% Cit.~\cite{Schneider2020} & 22 & \textbf{2.63\,k} & 223\,k & 12.98\,M & 71.30 \\
% Cit.~\cite{Schirrmeister2017DeepVisualization} & 22 & 47.3\,k & 1,013\,k & 63.0\,M & 74.31 \\
% Cit.~\cite{Hersche2018FastFeatures} & 22 & 261\,k & 50\,k & 104\,M & 73.70 \\
% Cit.~\cite{Hersche2018FastFeatures} & 22 & 50.0\,k & 49\,k & - & 74.77 \\
% Cit.~\cite{wu2019_MSFBCNN} & 22 & 155\,k & 5,775\,k & 202\,M & 75.80 \\
% Cit~\cite{ingolfsson2020eegtcnet} & 22 & 4.27\,k & 396\,k & 6.8\,M & \textbf{77.35} \\
% %Cit.~\cite{zhao_improvement_2017} & 22 & 220\,k & 499\,k & 18.2\,M & \textbf{81.10} \\
% %\multicolumn{1}{l|}{TPCT~\cite{li_novel_2020}} & 88.87 & 7.78\,M & 1.73\,G & 524\\
% %Cit.~\cite{Arpaia2021BCICompCS} & 22 & - & - & - & 64 \\ % they use fbcsp
% %\midrule
% %This work & 14 & 3.044\,k & 33.75\,k & 1.48\,M & 70.54 \\ 
% %\midrule
% %This work & 10 & 2.98\,k & 29.25\,k & 1.41\,M & 71.87 \\ 
% %Cit.~\cite{Arpaia2021BCICompCS} & 10 & - & - & - & 62 \\ % they use fbcsp
% \bottomrule
% %\multicolumn{5}{l}{\scriptsize\textsuperscript{*}Reproduced}%
% \end{tabular}
% \end{table}

==> 02_figures/T_quant_net_mod.tex <==
\begin{table}[!b]
\centering
\caption{Network modifications for quantization-aware training and deployment. Changes are written in italic and highlighted in grey.}
\label{tab:quantization_layers}
% \begin{tabular}{@{}|l|c|c|c|c|@{}}
% \toprule
% Layer                   & \textPhi\textsuperscript{1} & \textPhi\textsuperscript{1} & \textPhi\textsuperscript{1} & \textPhi\textsuperscript{1} \\ \midrule
% \multirow{7}{*}{Types} & DepthConv2d                                                 & DepthConv2d                                                 & DepthConv2d                                                 & FC                                                          \\
%                       & BatchNorm2d                                                 & BatchNorm2d                                                 & \textit{Quantization}                                       & SoftMaxAct                                                  \\
%                       & \textit{Quantization}                                       & \textit{ReluAct}                                            & Conv2d                                                      &                                                             \\
%                       &                                                             & AvgPool2d                                                   & BatchNorm2d                                                 &                                                             \\
%                       &                                                             & \textit{Quantization}                                       & \textit{ReluAct}                                            &                                                             \\
%                       &                                                             &                                                             & AvgPool2d                                                   &                                                             \\
%                       &                                                             &                                                             & \textit{Quantization}                                       &                                                             \\ \bottomrule
% \end{tabular}
% \end{table}

\begin{tabular}{|l|c|c|c|c|}
\hline
Layer                   & \textPhi\textsuperscript{1} & \textPhi\textsuperscript{2} & \textPhi\textsuperscript{3} & \textPhi\textsuperscript{4} \\ \hline
                        & DepthConv2d                                                 & DepthConv2d                                                 & DepthConv2d                                                 & FC                                                          \\ \cline{2-5} 
                        & BatchNorm2d                                                 & BatchNorm2d                                                 & \cellcolor[HTML]{EFEFEF}\textit{Quantization}               & SoftMaxAct                                                  \\ \cline{2-5} 
                        & \cellcolor[HTML]{EFEFEF}\textit{Quantization}               & \cellcolor[HTML]{EFEFEF}\textit{ReluAct}                    & Conv2d                                                      &                                                             \\ \cline{2-4}
                        &                                                             & AvgPool2d                                                   & BatchNorm2d                                                 &                                                             \\ \cline{3-4}
                        &                                                             & \cellcolor[HTML]{EFEFEF}\textit{Quantization}               & \cellcolor[HTML]{EFEFEF}\textit{ReluAct}                    &                                                             \\ \cline{3-4}
                        &                                                             &                                                             & AvgPool2d                                                   &                                                             \\ \cline{4-4}
\multirow{-7}{*}{Types} &                                                             &                                                             & \cellcolor[HTML]{EFEFEF}\textit{Quantization}               &                                                             \\ \hline
\end{tabular}
\end{table}




% \begin{tabular}{|l|c|c|c|c|}
% \hline
% Layer                  & \textPhi\textsuperscript{1} & \textPhi\textsuperscript{1} & \textPhi\textsuperscript{1} & \textPhi\textsuperscript{1} \\ \hline
% \multirow{7}{*}{Types} & DepthConv2d                                                 & DepthConv2d                                                 & DepthConv2d                                                 & FC                                                          \\ \cline{2-5} 
%                       & BatchNorm2d                                                 & BatchNorm2d                                                 & \textit{Quantization}                                       & SoftMaxAct                                                  \\ \cline{2-5} 
%                       & \textit{Quantization}                                       & \textit{ReluAct}                                            & Conv2d                                                      &                                                             \\ \cline{2-4}
%                       &                                                             & AvgPool2d                                                   & BatchNorm2d                                                 &                                                             \\ \cline{3-4}
%                       &                                                             & \textit{Quantization}                                       & \textit{ReluAct}                                            &                                                             \\ \cline{3-4}
%                       &                                                             &                                                             & AvgPool2d                                                   &                                                             \\ \cline{4-4}
%                       &                                                             &                                                             & \textit{Quantization}                                       &                                                             \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[!b]\label{tab:quantization}
% \centering
% \caption{Here}
% \begin{tabular}{@{}lr@{}}
% \toprule
% Layer                                                                         & Type                                          \\ \midrule
%                                                                               & DepthConv2d                                   \\
%                                                                               & BatchNorm2d                                   \\
% \multirow{-3}{*}{\textPhi\textsuperscript{1}} & \cellcolor[HTML]{EFEFEF}\textit{Quantization} \\
%                                                                               & DepthConv2d                                   \\
%                                                                               & BatchNorm2d                                   \\
%                                                                               & \cellcolor[HTML]{EFEFEF}ReluAct               \\
%                                                                               & AvgPool2d                                     \\
% \multirow{-5}{*}{\textPhi\textsuperscript{1}} & \cellcolor[HTML]{EFEFEF}\textit{Quantization} \\
%                                                                               & DepthConv2d                                   \\
%                                                                               & \cellcolor[HTML]{EFEFEF}\textit{Quantization} \\
%                                                                               & Conv2d                                        \\
%                                                                               & BatchNorm2d                                   \\
%                                                                               & \cellcolor[HTML]{EFEFEF}ReluAct               \\
%                                                                               & AvgPool2d                                     \\
% \multirow{-7}{*}{\textPhi\textsuperscript{1}} & \cellcolor[HTML]{EFEFEF}\textit{Quantization} \\
%                                                                               & FC                                            \\
% \multirow{-2}{*}{\textPhi\textsuperscript{1}} & \multicolumn{1}{l}{SoftMaxAct}                \\ \bottomrule
% \end{tabular}
% \end{table}

==> 02_figures/T_quant_res.tex <==
\begin{table}[!b]
\caption{32-bit full-precision vs. 8-bit quantized accuracy.}
\centering
\label{tab:quant_acc}
\begin{tabular}{@{}lrrrcrrr@{}}
\toprule
&\multicolumn{3}{c}{Physionet \gls{mmmi}} & & \multicolumn{3}{c}{BCI Comp. IV-2a} \\ 
\cmidrule(l){2-4} \cmidrule(l){6-8}
%\multicolumn{2}{c}{\#\,classes}                           
& 2-           & 3-           & 4-     &     & 2- & 3- & 4-class               \\
% \cmidrule(){1-2} \cmidrule(l){3-5} \cmidrule(l){6-6} 
\midrule
32-bit & 82.79       & 74.92       & 65.62   &   & 86.32 &  80.37    & 76.03      \\
8-bit  & 82.61       & 75.12       & 65.31    &   & &   &        \\ 
\bottomrule
\end{tabular}
\end{table}

%\begin{table}[!b]
% \caption{Quantized vs. full-precision accuracy.}
% \centering
% \label{tab:quant_acc}
% \begin{tabular}{@{}llcccc@{}}
% \toprule
% &  & \multicolumn{3}{c}{Physionet \gls{mmmi}} & BCI Comp. IV-2a \\ 
% \cmidrule(l){3-5} \cmidrule(l){6-6}
% %\multicolumn{2}{c}{\#\,classes}                           
% & & 2           & 3           & 4          & 4-class               \\
% % \cmidrule(){1-2} \cmidrule(l){3-5} \cmidrule(l){6-6} 
% \midrule
% \multicolumn{1}{l|}{\multirow{2}{*}{\edgeeegnet{}}}   & 32-bit & 82.79       & 74.92       & 65.62      & 72.60           \\
% \multicolumn{1}{l|}{}                        & 8-bit  & 82.61       & 75.12       & 65.31      & 71.71           \\ 
% \cmidrule(){1-2} \cmidrule(l){3-5} \cmidrule(l){6-6} %\midrule
% \multicolumn{1}{l|}{\multirow{2}{*}{\eegnet{}}} & 32-bit & 82.29       & 74.46       & 64.85      & 71.3~\cite{Schneider2020}            \\
% \multicolumn{1}{l|}{}                        & 8-bit  & 82.61       & 74.07       & 65.14      & 70.9~\cite{Schneider2020}            \\ \bottomrule
% \end{tabular}
% \end{table}
